Evaluated CMI Bounds for Meta Learning: Tightness and Expressiveness

Recent work has established that the conditional mutual information (CMI) framework of Steinke and Zakynthinou (2020) is expressive enough to capture generalization guarantees in terms of algorithmic stability, VC dimension, and related complexity measures for conventional learning (Harutyunyan et al., 2021, Haghifam et al., 2021). Hence, it provides a unified method for establishing generalization bounds. In meta learning, there has so far been a divide between information-theoretic results and results from classical learning theory. In this work, we take a first step toward bridging this divide. Specifically, we present novel generalization bounds for meta learning in terms of the evaluated CMI (e-CMI). To demonstrate the expressiveness of the e-CMI framework, we apply our bounds to a representation learning setting, with $n$ samples from $\hat n$ tasks parameterized by functions of the form $f_i \circ h$. Here, each $f_i \in \mathcal F$ is a task-specific function, and $h \in \mathcal H$ is the shared representation. For this setup, we show that the e-CMI framework yields a bound that scales as $\sqrt{ \mathcal C(\mathcal H)/(n\hat n) + \mathcal C(\mathcal F)/n} $, where $\mathcal C(\cdot)$ denotes a complexity measure of the hypothesis class. This scaling behavior coincides with the one reported in Tripuraneni et al. (2020) using Gaussian complexity.

==> tikzsettings.tex <==








\newcommand{\pop}[1]{\textcolor{OliveGreen}{#1}}

\newcommand{\popn}[1]{\textcolor{Apricot}{#1}}




\pgfkeys{tikz/mymatrixenv/.style={decoration={brace},every left delimiter/.style={xshift=8pt},every right delimiter/.style={xshift=-8pt}}}
\pgfkeys{tikz/mymatrix/.style={matrix of math nodes,nodes in empty cells,left delimiter={[},right delimiter={]},inner sep=1pt,outer sep=1.5pt,column sep=8pt,row sep=8pt,nodes={minimum width=20pt,minimum height=10pt,anchor=center,inner sep=0pt,outer sep=0pt}}}
\pgfkeys{tikz/mymatrixbrace/.style={decorate,thick}}
\pgfkeys{tikz/mymatrixbracethin/.style={decorate}}

\newcommand*\mymatrixbraceright[4][m]{
    \draw[mymatrixbrace] (#1.west|-#1-#3-1.south west) -- node[left=2pt, align = left] {#4} (#1.west|-#1-#2-1.north west);
}
\newcommand*\mymatrixbraceleft[4][m]{
    \draw[mymatrixbrace] (#1.east|-#1-#2-1.north east) -- node[right=2pt, align = center] {#4} (#1.east|-#1-#2-1.south east);
}
\newcommand*\mymatrixbracetop[4][m]{
    \draw[mymatrixbrace] (#1.north-|#1-1-#2.north west) -- node[above=2pt, align = center] {#4} (#1.north-|#1-1-#3.north east);
}
\newcommand*\mymatrixbracebottom[4][m]{
    \draw[mymatrixbrace] (#1.south-|#1-1-#2.north east) -- node[below=2pt, align = center] {#4} (#1.south-|#1-1-#3.north west);
}

\newcommand*\mymatrixbracetopShat[4][Shat]{
    \draw[mymatrixbrace] (#1.north-|#1-1-#2.north west) -- node[above=2pt, align = center] {#4} (#1.north-|#1-1-#3.north east);
}
\newcommand*\mymatrixbracebottomS[4][S]{
    \draw[mymatrixbrace] (#1.south-|#1-1-#2.north east) -- node[below=2pt, align = center] {#4} (#1.south-|#1-1-#3.north west);
}


\tikzset{style green/.style={
    set fill color=OliveGreen!50!lime!60,draw opacity=0.4,
    set border color=OliveGreen!50!lime!60,fill opacity=0.1,
  },
  style cyan/.style={
    set fill color=cyan!90!blue!60, draw opacity=0.4,
    set border color=blue!70!cyan!30,fill opacity=0.1,
  },
  style orange/.style={
    set fill color=orange!90, draw opacity=0.8,
    set border color=orange!90, fill opacity=0.3,
  },
  style brown/.style={
    set fill color=brown!70!orange!40, draw opacity=0.4,
    set border color=brown, fill opacity=0.3,
  },
  style purple/.style={
    set fill color=violet!90!pink!20, draw opacity=0.5,
    set border color=violet, fill opacity=0.3,    
  },
  style red/.style={
    set fill color=Red!90!pink!20, draw opacity=0.5,
    set border color=Red, fill opacity=0.3,    
  },
  Sh1/.style={
    above left offset={-0.08,0.25},
    below right offset={0.07,-0.16},
    #1
  },
  Sh/.style={
    above left offset={-0.07,0.25},
    below right offset={0.12,-0.16},
    #1
  },
  big/.style={
    above left offset={-0.01,0.375},
    below right offset={0.16,-0.35},
    #1
  },
  mid/.style={
    above left offset={-0.07,0.34},
    below right offset={0.12,-0.32},
    #1
  },
  small/.style={
    above left offset={-0.03,0.3},
    below right offset={0.09,-0.25},
    #1
  },set fill color/.code={\pgfkeysalso{fill=#1}},
  set border color/.style={draw=#1}
}
